TNM: A Tool for Mining of Socio-Technical Data from Git Repositories

Networks of collaboration between engineers are reflected in traces of developers' activity in version control systems (VCSs). Extracting data from Git repositories is an essential task for researchers and practitioners working on socio-technical analysis, but it requires substantial engineering work. With increasing interest in analysing socio-technical data and applying it in practice, there are no flexible and easily reusable tools to retrieve socio-technical information from VCSs. With no common reusable toolkit existing for this task, the burden of mining diverts the focus of researchers from their core research questions. In this paper, we present TNM -- an open-source tool for mining socio-technical data from Git repositories. TNM is fast, flexible, and easily extensible. TNM is available on GitHub: https://github.com/JetBrains-Research/tnm

==> sections/extraction_data_from_git.tex <==
\section{Extracting data from git repositories}
% cite https://git-scm.com/book/en/v2/Getting-Started-What-is-Git%3F
As mention before we getting all needed data from git repositories, 
which is commonly used in projects.
Git is version control tool with a snapshot data model. It basically
takes a picture of what all files look like at the moment and 
stores a reference to that snapshot. To be efficient, if files have
not changed, Git does not store the file again, just a link to the
previous identical file it has already stored. 

The main tools for mining data are commits. 
Commit stores saves files as they are and permanently stores
snapshot to your Git directory and has the following structure: 
\begin{itemize}
    \item A set of links to files in a git repository
    \item Link to parent commits
    \item Meta information (author, date, changed files etc.)
\end{itemize}
Going through the commit history of developers we extract needed 
data from meta information of commits. 
% write about diffs
By using that information, 
we can calculate dependencies between developers and project entities. Than we can visualize mined data as networks.
